Ergodic theorem and algorithmic randomness

We prove the constructive version of Birkhoff's ergodic theorem following Vyugin but trying to separate and state explicitly the combinatorial statement on which this proof is based. We pose some questions related to this statement (and the effective ergodic theorem in general).

==> pict/Makefile <==
pdf: ; \
  lualatex ergodic-1.tex;\
  lualatex ergodic-2.tex;\
  lualatex ergodic-3.tex;\
  lualatex ergodic-4.tex;\
  lualatex ergodic-5.tex;\
  rm *.log ;\
  rm *.aux ;\


clean: ; \
  rm *.pdf ;\
  rm *.log ;\
  rm *.aux ;\
  rm *.gz  ;\


==> pict/ergodic-1.tex <==
%!TEX TS-program = lualatex
%!TEX encoding = UTF-8 Unicode

\input lualib.tex
\begin{mplibcode}
numeric u; u=5mm;
numeric s; s=2u;

numeric alpha; alpha=-0.025;
numeric beta; beta=0.12;

beginfig(1)
f1=0.4u; f2=-0.8u; f3=u; f4=0.6u; f5=-u; f6=-0.4u; f7=2.1u; f8=-1.2u; f9=-0.7u;
numeric k; k=7s;
pair low; low=(k,alpha*k);
pair high; high=(k,beta*k);
path triangle; triangle=(0,0)--low--high--cycle;
z0=(0,0);
z1=(s,f1);
z2=z1+(s,f2);
z3=z2+(s,f3);
z4=z3+(s,f4);
z5=z4+(s,f5);
z6=z5+(s,f6);
z7=z6+(s,f7);
fill triangle withcolor 0.8[green+blue,white];
draw z0--low withcolor 0.8blue;
draw z0--high withcolor 0.8red;

for i = z0,z1,z2,z3,z4,z5,z6,z7:
  draw i withpen pencircle scaled 2pt;
endfor;
drawarrow z0--z1;
drawarrow z1--z2;
drawarrow z2--z3;
drawarrow z3--z4;
drawarrow z4--z5;
drawarrow z5--z6;
drawarrow z6--z7;
label.bot (btex $(0,0)$ etex, z0);
label.top (btex $(1,a_1)$ etex, z1);
label.bot (btex $(2,a_1+a_2)$ etex, z2);
label.top (btex $(k,a_1+\ldots+a_k)$ etex, z7);
label.rt (btex $\alpha$ etex, low);
label.rt (btex $\beta$ etex, high);
endfig;

\end{mplibcode}
\end{document}

==> pict/ergodic-2.tex <==
%!TEX TS-program = lualatex
%!TEX encoding = UTF-8 Unicode

\input lualib.tex
\begin{mplibcode}
numeric u; u=5mm;
numeric s; s=2u;

numeric alpha; alpha=-0.025;
numeric beta; beta=0.12;

beginfig(2)

f1=0.4u; f2=-0.8u; f3=u; f4=0.6u; f5=-u; f6=-0.4u; f7=2.1u; f8=-1.2u; f9=-0.7u;
numeric k; k=7s;
pair low; low=(k,alpha*k);
pair high; high=(k,beta*k);

def drawtriangle(expr u)=
  path triangle; triangle=(0,0)--low--high--cycle;
  fill triangle shifted u withcolor 0.8[green+blue,white];
enddef;

def drawbtriangle(expr u)=
  path triangle; triangle=(0,0)--low--high--cycle;
  draw (z0--low) shifted u withcolor 0.8blue;
  draw (z0--high) shifted u withcolor 0.8red;
enddef;

z0=(0,0);
z1=(s,f1);
z2=z1+(s,f2);
z3=z2+(s,f3);
z4=z3+(s,f4);
z5=z4+(s,f5);
z6=z5+(s,f6);
z7=z6+(s,f7);
z8=z7+(s,f8);
z9=z8+(s,f9);
drawtriangle(z0);
%drawtriangle(z1);
drawtriangle(z2);
drawbtriangle(z0);
%drawbtriangle(z1);
drawbtriangle(z2);
for i = z0,z1,z2,z3,z4,z5,z6,z7,z8,z9:
  draw i withpen pencircle scaled 2pt;
endfor;
drawarrow z0--z1;
drawarrow z1--z2;
drawarrow z2--z3;
drawarrow z3--z4;
drawarrow z4--z5;
drawarrow z5--z6;
drawarrow z6--z7;
drawarrow z7--z8;
drawarrow z8--z9;
endfig;


\end{mplibcode}
\end{document}

==> pict/ergodic-3.tex <==
%!TEX TS-program = lualatex
%!TEX encoding = UTF-8 Unicode

\input lualib.tex
\begin{mplibcode}
numeric u; u=5mm;
numeric s; s=2u;

numeric alpha; alpha=-0.025;
numeric beta; beta=0.12;

beginfig(2)

f1=0.4u; f2=-0.8u; f3=u; f4=0.6u; f5=-u; f6=-0.4u; f7=2.1u; f8=-1.2u; f9=-0.7u;
numeric k; k=7s;
pair low; low=(k,alpha*k);
pair high; high=(k,beta*k);

def drawtriangle(expr u)=
  path triangle; triangle=(0,0)--low--high--cycle;
  fill triangle shifted u withcolor 0.8[green+blue,white];
enddef;

def drawbtriangle(expr u)=
  path triangle; triangle=(0,0)--low--high--cycle;
  draw (z0--low) shifted u withcolor 0.8blue;
  draw (z0--high) shifted u withcolor 0.8red;
enddef;

z0=(0,0);
z1=(s,f1);
z2=z1+(s,f2);
z3=z2+(s,f3);
z4=z3+(s,f4);
z5=z4+(s,f5);
z6=z5+(s,f6);
z7=z6+(s,f7);
z8=z7+(s,f8);
z9=z8+(s,f9);

for i = z0,z1,z2,z3,z4,z5,z6,z7,z8,z9:
  draw i withpen pencircle scaled 2pt;
endfor;
drawarrow z0--z1 withpen pencircle scaled 1.2pt;
drawarrow z1--z2 dashed evenly;
drawarrow z2--z3 withpen pencircle scaled 1.2pt;
drawarrow z3--z4 withpen pencircle scaled 1.2pt;
drawarrow z4--z5 dashed evenly;
drawarrow z5--z6 dashed evenly;
drawarrow z6--z7 withpen pencircle scaled 1.2pt;
drawarrow z7--z8 dashed evenly;
drawarrow z8--z9 dashed evenly;
endfig;


\end{mplibcode}
\end{document}

==> pict/ergodic-4.tex <==
%!TEX TS-program = lualatex
%!TEX encoding = UTF-8 Unicode

\input lualib.tex
\begin{mplibcode}
numeric u; u=5mm;
numeric s; s=2u;

numeric alpha; alpha=-0.025;
numeric beta; beta=0.12;

beginfig(1)

f1=0.4u; f2=-0.8u; f3=u; f4=0.6u; f5=-u; f6=-0.4u; f7=2.1u; f8=-1.2u; f9=-0.7u;
numeric k; k=7s;
numeric axis; axis=-2u;

z0=(0,0);
z1=(s,f1);
z2=z1+(s,f2);
z3=z2+(s,f3);
z4=z3+(s,f4);
z5=z4+(s,f5);
z6=z5+(s,f6);
z7=z6+(s,f7);
z8=z7+(s,f8);
z9=z8+(s,f9);

for i = z0,z1,z2,z3,z4,z5,z6,z7,z8,z9:
  draw i withpen pencircle scaled 2pt;
endfor;
for i = z0,z1,z2,z4,z6,z7:
  draw i withpen pencircle scaled 2pt;
  pair ii; 
  ii = (whatever,axis)=i+(0,whatever);
  draw ii--i;
  draw ii withpen pencircle scaled 1.2pt;
endfor;
draw (0,axis)--(9s,axis);
drawarrow z0--z1 withpen pencircle scaled 1.2pt;
drawarrow z1--z2 dashed evenly;
drawarrow z2--z3 withpen pencircle scaled 1.2pt;
drawarrow z3--z4 withpen pencircle scaled 1.2pt;
drawarrow z4--z5 dashed evenly;
drawarrow z5--z6 dashed evenly;
drawarrow z6--z7 withpen pencircle scaled 1.2pt;
drawarrow z7--z8 dashed evenly;
drawarrow z8--z9 dashed evenly;

label.bot(btex $l_1$ etex, (0,axis));
label.bot(btex $r_1$ etex, (s,axis));
label.bot(btex $l_2$ etex, (2s,axis));
label.bot(btex $r_2$ etex, (4s,axis));
label.bot(btex $l_3$ etex, (6s,axis));
label.bot(btex $r_3$ etex, (7s,axis));
endfig;



\end{mplibcode}
\end{document}

==> pict/ergodic-5.tex <==
%!TEX TS-program = lualatex
%!TEX encoding = UTF-8 Unicode

\input lualib.tex
\begin{mplibcode}
numeric u; u=5mm;
numeric s; s=2u;

numeric alpha; alpha=-0.025;
numeric beta; beta=0.12;

beginfig(1)

f1=-0.4u; f2=0.8u; f3=-1.1u; f4=2.2u; f5=-2.3u; f6=1.1u; f7=0.2u; 
numeric k; k=7s;
pair low; low=(k,alpha*k);
pair high; high=(k,beta*k);

def drawtriangle(expr u)=
  path triangle; triangle=(0,0)--low--high--cycle;
  fill triangle shifted u withcolor 0.8[green+blue,white];
enddef;

def drawbtriangle(expr u)=
  path triangle; triangle=(0,0)--low--high--cycle;
  draw (z0--low) shifted u withcolor 0.8blue;
  draw (z0--high) shifted u withcolor 0.8red;
enddef;

z0=(0,0);
z1=(s,f1);
z2=z1+(s,f2);
z3=z2+(s,f3);
z4=z3+(s,f4);
z5=z4+(s,f5);
z6=z5+(s,f6);
z7=z6+(s,f7);
drawtriangle(z0);
drawbtriangle(z0);
for i = z3,z4,z5:
  draw i withpen pencircle scaled 2pt;
endfor;
draw z0{right}...z1...z2...z3...z4...z5...z6...z7;
numeric axis; axis=-1.2u;

pair a,b,c;
pair aa,bb,cc;
a = z3+(0,whatever) = (whatever,axis);
aa=z3+(0,whatever)=whatever*low;
draw z3--a;
draw z3--aa withpen pencircle scaled 1.2pt;
b = z4+(0,whatever) = (whatever,axis);
bb=z4+(0,whatever)=whatever*high;
draw z4--b;
draw z4--bb withpen pencircle scaled 1.2pt;
c = z5+(0,whatever) = (whatever,axis);
cc=z5+(0,whatever)=whatever*low;
draw z5--c;
draw z5--cc withpen pencircle scaled 1.2pt;
label.bot (btex $\mathstrut u$ etex, a);
label.bot (btex $\mathstrut v$ etex, b);
label.bot (btex $\mathstrut w$ etex, c);
endfig;




\end{mplibcode}
\end{document}
